Meta-Learning with Graph Neural Networks: Methods and Applications

Graph Neural Networks (GNNs), a generalization of deep neural networks on graph data have been widely used in various domains, ranging from drug discovery to recommender systems. However, GNNs on such applications are limited when there are few available samples. Meta-learning has been an important framework to address the lack of samples in machine learning, and in recent years, researchers have started to apply meta-learning to GNNs. In this work, we provide a comprehensive survey of different meta-learning approaches involving GNNs on various graph problems showing the power of using these two approaches together. We categorize the literature based on proposed architectures, shared representations, and applications. Finally, we discuss several exciting future research directions and open problems.

==> 7_new_papers.tex <==

\clearpage
\section{New papers}

\subsection{Anomaly detection}


\begin{itemize}
    \item \textbf{Few-shot Network Anomaly Detection via Cross-network Meta-learning \cite{ding_www21}}: The problem of anomaly detection often suffers from scarcity of labels. To obtain labels for anomalies is usually labor intensive. Many existing methods are developed in unsupervised manner. Others (auto-encoder, matrix factorization based) lack prior knowledge on anomalies of interest. A potential approach could leverage a few labeled anomalies \cite{ding_www21} to build a prior knowledge about them. \citet{ding_www21} study anomaly detection when there are scarcity of labels. The different tasks involve different graphs. The proposed method used traditional GNN architecture to embed nodes and predict the anomaly score by adding another layer after the embedding is obtained. Finally it  exploits the traditional MAML framework to deploy the meta-learner. The inner loop optimizes the parameters for a specific task, i.e., graph. The outer-loop optimizes the generic parameter for all graphs.
\end{itemize}



\subsection{Node Classification}

\begin{itemize}
\item \textbf{Meta-Inductive Node Classification  across Graphs \cite{wen2021meta}}:  \citet{wen2021meta} studied the problem of node classification in an inductive setting. The graph instances in meta testing and training do not overlap. Their method involves computing a task prior given a graph (i.e., its representation) using MLPs. These help in graph-level adaptation. They also used the traditional MAML paradigm in their approach for task-level adaptation. 


\item \textbf{Weakly-supervised Graph Meta-learning for Few-shot Node Classification \cite{ding2021weakly}:}
The idea is to perform few-shot node classification tasks with the presence of noisy or inaccurate labels in the support sets of different tasks. \citet{ding2021weakly} proposed a method (Graph Hallucination Network) that creates a set by taking a specified number of samples from a class. Then the method learns to produce a confidence score on the accuracy of the label of each node in the set. By using these weights/scores, the final cleaner (i.e., less noisy) node representations are generated. The rest of the algorithm follows a standard MAML framework. 
\end{itemize}

\subsection{Graph Classification}
\begin{itemize}
    \item \textbf{Structure-Enhanced Meta-Learning For Few-Shot Graph Classification \cite{jiang2021structure}}:
\citet{jiang2021structure} solved the problem of few shot graph classification via a paradigm in meta learning called metric learning approach \cite{wang2019simpleshot} that is different from MAML. In the training phase, the idea is to get a mean representations of the instances in each class in the support set. The prediction for query is based on the nearest neighbour. Here the graph representations were obtained by the GIN model. To capture the global structure of the graph, they used different weights for different GIN layers in the final aggregation scheme. To encode the crucial local structures that might have importance ind deciding the graph label, the paper embed subgraphs and include their representations with different attention weights. 
\end{itemize}


\subsection{Node Classification and Link Prediction}
\begin{itemize}
    \item \textbf{Self-supervised Auxiliary Learning for Graph Neural Networks via Meta-Learning \cite{hwang2021self}}: 
    In this paper, \citet{hwang2021self} studies the effectiveness of graph neural networks on downstream tasks such as node classification and link prediction via a self-supervised auxiliary learning framework combining with meta-learning. The framework is shown to be effective on heterogeneous graphs. The auxiliary tasks involve task such as meta-path prediction which does not need labels and thus the method becomes self-supervised. In the meta learning framework, various auxiliary tasks had been used to improve generalization performance of the underlying primary task (e.g., link prediction). The proposed method effectively combines the auxiliary tasks and automatically balances them to improve performance on the primary task. The method is also flexible to work with any graph neural network architecture without additional data.

\end{itemize}
